A Framework for Efficient Model Evaluation through Stratification, Sampling, and Estimation

Model performance evaluation is a critical and expensive task in machine learning and computer vision. Without clear guidelines, practitioners often estimate model accuracy using a one-time completely random selection of the data. However, by employing tailored sampling and estimation strategies, one can obtain more precise estimates and reduce annotation costs. In this paper, we propose a statistical framework for model evaluation that includes stratification, sampling, and estimation components. We examine the statistical properties of each component and evaluate their efficiency (precision). One key result of our work is that stratification via k-means clustering based on accurate predictions of model performance yields efficient estimators. Our experiments on computer vision datasets show that this method consistently provides more precise accuracy estimates than the traditional simple random sampling, even with substantial efficiency gains of 10x. We also find that model-assisted estimators, which leverage predictions of model accuracy on the unlabeled portion of the dataset, are generally more efficient than the traditional estimates based solely on the labeled data.

==> macros/macros-pp.tex <==
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}

\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}}
\newcommand{\argmax}{\mathop{\mathrm{arg\,max}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}
\newcommand{\maximize}{\mathop{\mathrm{maximize}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\Var}{{\mathop{\mathrm{Var}}}}
\newcommand{\Bias}{{\mathop{\mathrm{Bias}}}}
\newcommand{\Cov}{{\mathop{\mathrm{Cov}}}}
\newcommand{\op}{\mathop{op}}

\newcommand{\mse}{\mathrm{MSE}}

\renewcommand{\bar}{\overline}

\renewcommand{\tilde}{\widetilde}

\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}

\newcommand{\asto}{\xrightarrow{\textup{a.s.}}}
\newcommand{\pto}{\xrightarrow{\textup{p}}}
\newcommand{\dto}{\xrightarrow{\textup{d}}}

\newcommand{\frr}{\mathtt{FRR}}
\newcommand{\far}{\mathtt{FAR}}

\renewcommand{\hat}{\widehat}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\gray}[1]{{\color{gray}#1}}
\newcommand{\brown}[1]{{\color{brown}Maybe to add: #1}}



==> miscellaneous/temporary.tex <==
\section{Temporary notes}
% https://aideadlin.es/?sub=ML,CV,NLP,RO,GR
% https://aideadlin.es/conference/?id=aistats24
% https://aideadlin.es/conference/?id=cvpr24

TODO: can we use ensemble classifiers?
TODO: Is the optimal allocation based on a wrong model vs. proportional allocation in the first step? Does monotonic scores matter?

\subsection*{Setup and terminology}

\begin{itemize}
    \item True safe, true danger
    \item Predicted safe, predicted danger
    \item We look into the predicted safe prompts
    \item Within predicted safe prompts, we want to figure out what prompts to select to ask humans for ``ground truths''
    \item Using these ``ground truths'', we wish to figure the true ``false safe'' rate
    \item ``False safe'' rate is the proportion of safe prompts which turn out to be danger
    \item Setup:
    \begin{itemize}
        \item Look at all the predicted safe prompts
        \item Within that set, we have scores from the algorithm
        that predicts how dangerous the prompt is.
        Suppose higher score means more dangerous
        \item Rank the prompts according to their danger.
        \item What we are really after is the probability that a randomly sampled predicted safe prompt is actually true danger?
        \item For simplicity assume that we have enough predicted safe prompts that we know this population.
        \item A naive strategy is just many prompts the set of predicted safe prompts, get the true labels, and compute this probability.
        \item But we want to do this efficiently given a certain number of queries.
        \item Let the number of predicted safe prompts be $n$. Let the budget of available queries to be $k$.
        \item We will make a simple model that there are two groups of predicted safe prompts: Those with high predicted scores ($s$=1) and those with low scores ($s$=0). 
        \item The distinguishing factor between the groups is the false safe rate. This is probability of label being true danger for a randomly sampled prompts from these groups.
        \item Let these false safe rates be $p_{s=1}$ and $p_{s=0}$.
        \item The true false safe rate is $d_{s=1} p_{s=1} + d_{s=0} p_{s=0}$ where $d_{s=1}$ is empirical fraction of high score predicted safe prompts and $d_{s=0}$ is the empirical fraction of low score prompts. Note that $d_{s=1} + d_{s=0} = 1$.
        \item Objective is to figure out $k_{s=1}$ and $k_{s=0}$ such that we randomly sample $k_{s=1}$ prompts from the high score group and $k_{s=0}$ prompts from the low score group.
        \item Once we sample respective prompts, the estimators for false safe rates within each groups are simply computed as empirical averages.
    \end{itemize}
\end{itemize}

\subsection*{Derivation of optimal allocation}

For simplicity of notation, in the below we denote:
$d_h$, $p_h$, and $\hat{p}_h$.
Similarly, for the low score group.

The general estimator looks like:
\begin{equation}
    \hat p = d_h \hat p_h + d_l \hat p_l. 
\end{equation}
% where 
% \begin{equation}
%     \hat p_h = \frac{1}{k_h} \sum_{i=1}^{k_h} 
% \end{equation}

Note that:
\begin{equation}
    \EE[\hat p_h] = p_h, \; \Var(\hat p_h) = \frac{p_h(1-p_h)}{k_h}. 
\end{equation}
Similarly for the low score group.

We will now compute the bias and variance of the proposed estimator.
\begin{equation}
    \EE[\hat p] = d_h p_h + d_{\ell} p_{\ell} = p.
\end{equation}

\begin{equation}
    \Var(\hat p) 
    = d_h^2 \frac{p_h(1-p_h)}{k_h} + d_l^2 \frac{p_l(1-p_l)}{k_l}
    = d_h^2 \frac{p_h(1-p_h)}{k_h} + d_l^2 \frac{p_l(1-p_l)}{k - k_h}.
\end{equation}

Now, we want to minimize the expression above. 
We will first write $k_l = k - k_h$ so that the only variable is $k_h$.
Then we will pretend it is a real variable without any constraints.
In particular, we will not constrain it to lie between $0$ and $k$ initially.
Once we get the answer, we will verify that this is indeed satisfied.
We will perform the unconstrained optimization by simply finding the stationary point of the objective function.
We do this by setting derivative with respect to $k_h$ to be $0$.
\begin{align}
\frac{\mathrm d}{\mathrm d {k_h}} \left\{d_h^2 \frac{p_h(1-p_h)}{k_h} + d_l^2 \frac{p_l(1-p_l)}{k - k_h} \right\}  = 0\\
\implies - d_h^2 \frac{p_h(1-p_h)}{k_h^2} + d_l^2 \frac{p_l(1-p_l)}{(k - k_h)^2} = 0 \\
\implies d_h^2 \frac{p_h(1-p_h)}{k_h^2} = d_l^2 \frac{p_l(1-p_l)}{(k - k_h)^2} \\
\implies d_h \frac{\sqrt{p_h(1-p_h)}}{k_h} = d_l \frac{\sqrt{p_l(1-p_l)}}{(k - k_h)} \\
\implies
\frac{k - k_h}{k_h}
= \frac{d_l}{d_h} \frac{\sqrt{p_l (1 - p_l)}}{\sqrt{p_h (1 - p_h)}} \\
\implies
\frac{k_l}{k_h} - 1
= \frac{d_l}{d_h} \frac{\sqrt{p_l (1 - p_l)}}{\sqrt{p_h (1 - p_h)}} \\
\implies
d_h \frac{\sqrt{p_h (1-p_h)}}{k_h}
= d_l \frac{\sqrt{p_l (1-p_l)}}{k_l}\\
\implies k_h = \frac{d_h\sqrt{p_h(1-p_h)}}{d_h \sqrt{p_h(1-p_h)} + d_l \sqrt{p_l(1-p_l)}}k. 
\end{align}


General pattern in more bins is going to be that we match weighted variance of all the groups, meaning $d_h \sqrt{\Var({\hat p})}$ should be the same among all the groups.

Some observations regarding the allocation:

\begin{itemize}
    \item The higher the density of the group, the higher the samples.
    \item The higher the variance, the higher the samples.
    \item So the fraction is proportional to the product of density and square root of variance.
\end{itemize}

This allocation is called Neyman allocation.

\subsection*{Implementation of optimal allocation}

How do we implement Neyman allocation:

\begin{enumerate}
    \item Stratification:
    We want to stratify the reported safe prompts into different strata based on some homogeneity criterion.
    \item Calculate stratum variance
    \item Allocate samples
    \item Random sampling
\end{enumerate}

Take the entire set and do proportional allocation here. You get some false safe rate, which will be pretty high. 
Somebody chooses a threshold for deployment so that the estimated $\hat p$ to match the desired target. 
Then start with the algorithm (you already done the first step). 
Proposed algorithm: repeat the following steps until annotation budget is exhausted. 
\begin{itemize}
    \item Compute initial mapping from scores onto probabilities. Potentially change the threshold. 
    \item Compute mapping from scores into variances
    \item Bin variances into G bins. How to choose G? Trade-off between making the allocation easier (at least one observation in each bin) and the grid fine-grained. Determined by $k$. 
    \item \textcolor{red}{Find strata of scores based on the variance bins}
    \item Compute the allocation using Neyman allocation
    \item Compute the false rates in each of the bins
    \item Update the scores with the false rates
    \item Repeat all operations (use the labels collected to update the mapping)
\end{itemize}




Some remarks:

\begin{itemize}
    \item The mapping is only used for allocation.
    So a suboptimal mapping can only make the sampling suboptimal.
    \item Once we sample, we always stay unbiased.
    \item We are not doing any worse than either simple random sample or proportional sample, provided that we eventually get a good estimate for the variances.
    \item If the variances happen to be homogeneous, then this strategy will become the proportional sampling.
    Proportional sampling may in turn become simple random sample in a large sample limit.
\end{itemize}




TODO: estimate cost savings


\subsection*{Sampling strategies overview}

A significant part of the error rate calibration process is the allocation of samples into the various strata. 
Two primary approaches are: the proportional and the optimal allocation methods. While the proportional sampling method aims to distribute samples evenly across all strata, the optimal allocation method uses variance information to allocate samples efficiently.

Despite the argument that the percentage of samples allocated to one stratum does not necessarily have to be optimal to maintain precision, according to (5.3) of \cite{cochran1977sampling}, the choice of strategy should consider the specific context.
A starting point could be proportional sampling, with modifications incorporated as more samples are collected and the characteristics of the data become clearer.

How to choose between optimal and proportional allocation. 
Some discussion in (5.10) of \cite{cochran1977sampling}.

\subsection*{Other methodologies}

\begin{itemize}[leftmargin=7mm]
    \item 
    The Dalenius-Hodges method serves as an effective tool to define strata boundaries, albeit with a few assumptions about the outcome. 
    One significant assumption is that the values of the outcome are known, a premise which is often impractical in real-world scenarios. 
    However, an effective workaround could be assuming that model predictions are well-calibrated for defining these boundaries.
    \item
    The geometric approach by Gunning and Horgan offers an alternative method for defining strata boundaries. 
    This approach provides a more flexible method to accommodate the intricacies of large-scale datasets and it would be beneficial to think about a similar approach.
    Reference: \url{https://www150.statcan.gc.ca/n1/pub/12-001-x/2004002/article/7749-eng.pdf}, \url{https://2011.isiproceedings.org/papers/650259.pdf}
\end{itemize}

\subsection*{Computing libraries}

\begin{itemize}[leftmargin=7mm]
    \item \url{http://repository.usp.ac.fj/12410/1/stratifyR_2020.pdf}
    \item \url{https://cran.r-project.org/web/packages/stratification/index.html}
\end{itemize}

\subsection*{Things to discuss}

We should discuss the methods above for defining strata versus using a grid of bins with same width versus other methods (I can run some experiments tomorrow), as well as how to compute false positive/negative rates and AUC efficiently. 

\subsection*{Algorithm to efficiently compute and calibrate error rates}

Input: model scores on a huge dataset, error metrics (canonical one is false safe), threshold for their current split to declare safe and danger

Output: estimated error metric using a given number of queries (say, 1000) for ground truths

Assume we have a way to map scores to true probability of safe or danger.
At any threshold, one can integrate the curve to find the true false safe rate.

Goodness: Suppose all methods are based on stratified sampling. Suppose we fix also the number of strata (how to figure this out is also interesting, but let's say we choose it somehow). So the only choice we have is: how do we allocate the given queries to different stratas. Then we can measure how optimal allocation with knowledge of ground truth data compares to other allocation. Having the groud truths allows you to compute the correct variance and hence get the true optimal allocation.

Assume that the true mapping from scores to true safe/danger probabiliites are monotonic.

\begin{itemize}
    \item Step 0: We start with assuming that the naive mapping from scores (which are assumed to be between $0$ and $1$) to safe/danger probabilities are correct. (Initialization; this will give us the current best guess for the probabilities; this also gives us the best guess for predicted variance)
    This just means that we have an identity map between scores and probabilities.
    \item Step 1: You can stratify based on predicted variance. (Strata allocation) These range from $0$ and $0.25$. Uniformly partition the variance.
    Cumulative square root for forming strata (page 38 of \url{https://beckassets.blob.core.windows.net/product/readingsample/9535345/9780198566625_excerpt_001.pdf}) \citep{dalenius1959minimum}
    \item Step 2: Now we allocate the given number of queries somehow. (Allocation component)
    At this point, we have a bunch of ground truths for some examples in the strata.
    \item Step 3: Within each group, we will now estimate the true danger probability. (Estimation component) Be careful about what exactly we estimate for each group.
    \item Step 3: (Calibration component)
\end{itemize}


Fix the number of strata, vary the strata boundaries and the allocation to each stratum

\subsection*{August 02, 2023}

We need to look at a bunch of real-world datasets and argue that the methods we are proposing are necessary and would greatly reduce the number of annotations needed (quantify in terms of money)

\begin{itemize}
    \item Initial strata allocation:
    partition the score range uniformly
    Currently done using Dalenius and Hodges (1995).
    \item $\Var(\hat{\Var}(\hat p) $ is upper bounded by $1/2(1 - 1/\sqrt{3})/n$ obtained via
    the Delta method
    \item Only use estimated probabilities to compute the optimal allocation if the standard error of the plug-in estimator is reasonable, i.e., below TK
    \item Soft switch versus hard  switch
    \item Compute expected gain and opportunity cost of switching vs. not switching
    \item proportional allocation: 
\end{itemize}

\subsection*{Rough calculations}

There are two stratas and we consider two steps.
In the first step, we perform proportional allocation.
In the second step, we compare whether to do proportional versus optimal allocation.

In total, we have $n$ to allocate in the second step.
From the first step, we have estimated $\hat{p}_1$ and $\hat{p}_2$.
This provides us with estimated square-root variances as $\hat{\sigma_1}$ and $\hat{\sigma_2}$.
If we knew the true $\sigma_1$ and $\sigma_2$, then the calculation that we have done above will show that the Neyman allocation is optimal.
The calculation below tries to see what happens by using $\hat{\sigma}_1$ and $\hat{\sigma}_2$.

For proportional allocation with two strata (1,2), for a sample size of $n$
\begin{equation}
    \Var(\bar{X}_{prop}) = \frac{p_1 \sigma_1^2 + p_2 \sigma_2^2}{n}
\end{equation} 

For optimal allocation, 
\begin{gather}
    \Var(\bar{X}_{opt}) = p_1^2 \frac{\sigma_1^2}{n\frac{p_1\hat\sigma_1}{p_1\hat\sigma_1 + p_2\hat\sigma_2}} + p_2^2 \frac{\sigma_2^2}{n\frac{p_2\hat\sigma_2}{p_1\hat\sigma_1 + p_2\hat\sigma_2}}\\
    = \frac{1}{n} \left( p_1\frac{\sigma_1^2}{\hat\sigma_1} + p_2\frac{\sigma_2^2}{\hat\sigma_2}\right)(p_1\hat\sigma_1 + p_2\hat\sigma_2)\\
    = \frac{1}{n} \left( p_1^2\sigma_1^2 + p_2^2\sigma_2^2 + p_1p_2\frac{\sigma_1^2\hat\sigma_2}{\hat\sigma_1}  + p_1p_2\frac{\sigma_2^2\hat\sigma_1}{\hat\sigma_2} \right) 
\end{gather}

It is worth noting that if $\hat{\sigma}_1 = \sigma_1$ and $\hat{\sigma}_2 = \sigma_2$, then the variance above for the optimal allocation is the optimal variance.
Also, if $\sigma_1 = \sigma_2$, then the optimal variance for the optimal allocation matches with the variance of the proportional allocation.

The only source of randomness in the variance for optimal allocation is the ratio $\hat{\sigma}_1 / \hat{\sigma}_2$.


We are interested in the likelihood that the variance under the second allocation is lower than the variance under proportional allocation. 
\begin{gather}
\mathbb{P}(\Var(\bar{X_{opt}}) \leq \Var(\bar{X_{prop}})) \\
\mathbb{P}\left(p_1^2\sigma_1^2 + p_2^2\sigma_2^2 + p_1p_2\frac{\sigma_1^2\hat\sigma_2}{\hat\sigma_1}  + p_1p_2\frac{\sigma_2^2\hat\sigma_1}{\hat\sigma_2}  \leq p_1 \sigma_1^2 + p_2 \sigma_2^2 \right)  \\
= \mathbb{P}\left(p_1p_2\frac{\sigma_1^2\hat\sigma_2}{\hat\sigma_1} + p_1p_2\frac{\sigma_2^2\hat\sigma_1}{\hat\sigma_2}\leq p_1 \sigma_1^2 + p_2 \sigma_2^2 -(p_1^2\sigma_1^2 + p_2^2\sigma_2^2) \right)\\
= \mathbb{P}\left(\frac{\sigma_1^2\hat\sigma_2}{\hat\sigma_1} + \frac{\sigma_2^2\hat\sigma_1}{\hat\sigma_2}\leq \frac{p_1 \sigma_1^2 + p_2 \sigma_2^2 -(p_1^2\sigma_1^2 + p_2^2\sigma_2^2)}{p_1p_2} \right)
\end{gather}
We wish to find how the number of instances allocated to estimating $\hat\sigma_1$ and $\hat\sigma_2$ depends on the underlying quantities. 

The idea is to compute an estimate for this probability using plug-in quantities.
This is probability is approximately (because of the Normal approximation)
\begin{equation}
    \mathbb{P}
    \left(
    \sigma_1^2 \frac{\cN(\sigma_2, 0.25/n_2)}{\cN(\sigma_1, 0.25/n_1)}
    + \sigma_2^2 \frac{\cN(\sigma_1, 0.25/n_1)}{\cN(\sigma_2, 0.25/n_2)}
    \le \frac{p_1 \sigma_1^2 + p_2 \sigma_2^2 -(p_1^2\sigma_1^2 + p_2^2\sigma_2^2)}{p_1p_2}
    \right)
\end{equation}
\textcolor{red}{what is a good estimator for the probability above?}
This still involves parameters that we do not know.
We then use the plug-in estimators for those parameters.
% The variance of a ratio estimator is given by \url{https://www.stat.cmu.edu/~hseltman/files/ratio.pdf}. 
% Here, this means that 
% \begin{gather}
        
% \end{gather}
We are essentially computing an estimate for the probability that the optimal allocation using empirical variance produces worse variance than the proportional allocation.

We want $\hat{\sigma}_1 / \hat{\sigma}_2$ to be close to $\sigma_1 / \sigma_2$.
In other words, we need the ratio of estimated standard errors to be close to the true ratio of standard deviations.

\begin{equation}
    \Var(\bar{X}_{prop}) - \Var(\bar{X}_{opt}) =  \frac{1}{n}(p_1(\sigma_1 - \bar{\sigma})^2 + p_2(\sigma_2 - \bar{\sigma})^2) 
\end{equation}
where $\bar{\sigma}=p_1\sigma_1 + p_2\sigma_2$. 

We are okay so long as:
\[
    \sigma_1^2 
    \left( \frac{\hat{\sigma}_2}{\hat{\sigma}_1} 
    - \frac{\sigma_2}{\sigma_1} \right)
    + \sigma_2^2 \left( \frac{\hat{\sigma}_1}{\hat{\sigma}_2}
    - \frac{\sigma_1}{\sigma_2} \right)
\]
is small.
This quantity is approximately unbiased, but has some variance.
We want to keep this quantity is small.
We simply compute an estimate for the variance (and may be also bias) of this quantity, and use that as a way to 


The distribution of $\hat{\sigma}_1$ is $\cN(\sigma_1, p_1 (1 - p_1) (1 - 2 p_1)^2 / n_1)$.


\subsection*{False positive and false negative rates}

So far, we have considered different ways of allocations for computing accuracy metrics.
Now, we consider allocations for computing false positive and false negative rates.

The main difference to the setting above is that we do not know the true density values.
This will need to be estimated.
The other challenge for optimal allocation is knowing the variances.

Below we start by computing the variance of estimator for false positive rate.
% https://www.stat.cmu.edu/~hseltman/files/ratio.pdf

We will assume we have strata.
We also assume that we have the right densities.
We need to know the variance of the estimated false positive and false negative rates within the strata.

\begin{gather}
    \Var\left( \frac{\hat\fp}{\hat\fp + \hat\tn} \right)  = \frac{\fp^2}{(\fp + \tn)^2} \left[ \frac{\Var(\hat\fp)}{\fp^2} - 2 \frac{\Cov(\hat\fp, \hat\fp + \hat\tn)}{\fp (\fp + \tn)} + \frac{\Var(\hat\fp + \hat\tn)}{(\fp + \tn)^2} \right]
\end{gather}
where
\begin{gather}
    \Cov(\hat\fp, \hat\fp + \hat\tn) = \Var(\hat\fp) + \Cov(\hat\fp, \hat\tn) = \Var(\hat\fp) + \Cov(\hat\fp, \hat\tn). 
\end{gather}

Then 
\begin{gather}
    \Var\left( \frac{\hat\fp}{\hat\fp + \hat\tn} \right) = \frac{\fp^2}{(\fp + \tn)^2} \left[ \frac{\Var(\hat\fp)(\tn - \fp)}{\fp^2(\fp + \tn)} + \frac{\Var(\hat\fp + \hat\tn)}{(\fp + \tn)^2} -2 \frac{\Cov(\hat\fp , \hat\tn)}{\fp (\fp + \tn)} \right]\\
    = \frac{\fp^2}{n(\fp + \tn)^2} \left[ \frac{\fp (1 - \fp) (\tn - \fp)}{\fp^2(\fp + \tn)} + \frac{(\fp + \tn) (1 - \fp - \tn)}{(\fp + \tn)^2} +2 \frac{\fp\cdot \tn}{\fp (\fp + \tn)} \right].
\end{gather}
% Thus, we have 
% \begin{gather}
%     \Var\left( \frac{\hat\fp}{\hat\fp + \hat\tn} \right) = 
% \end{gather}

Overall goal here is to get a reasonable estimator for the variance.

Our estimator for false positive rate, where proportions $p_1$ and $p_2$ are densities for each of the group:
\begin{gather}
    FPR = \frac{\fp_{1} + \fp_2}{\fp_1 + \tn_1 + \fp_2 + \tn_2}  \\
    = \frac{\fp_{1}}{\fp_1 + \tn_1}\frac{\fp_1 + \tn_1}{\fp + \tn} +   \frac{\fp_2}{\fp_2 + \tn_2}\frac{\fp_2 + \tn_2}{\fp + \tn} \label{eq:weighted-def-fp}
\end{gather}
hence an estimator is given by 
\begin{gather}
    \hat{FPR} = \frac{\hat\fp_{1} + \hat\fp_2}{\hat\fp_1 + \hat\tn_1 + \hat\fp_2 + \hat\tn_2}. 
\end{gather}
Then, how can we estimate $\hat\fp_1$ and $\hat\tn_1$? One estimator is 
\begin{gather}
    \hat\fp_1 = \frac{\sum_{i=1}^n (1 - y_i) 1(s=1) 1(b_i=1)}{\sum_{i=1}^n (1 - y_i)1(b_i=1)}N_1\\
    \hat\fp_1 + \hat\tn_1 = \sum_{i=1}^n (1 - y_i)1(b_i=1) N_1
\end{gather}
where $N_1 = \sum_{i=1}^n 1(b_i = 1)$. 

\begin{align}
    &\Var(\hat\fpr^{prop}) - \Var(\hat\fpr^{srs}) \\
    &= \sum_{i=1}^d \Var(\hat\fpr_i) \frac{(\fp_i + \tn_i)^2}{(\fp + \tn)^2} - \sum_{i=1}^d \frac{(\fp_i + \tn_i)}{(\fp + \tn)}\Var(\hat\fpr^{srs})\\
    &= \sum_{i=1}^d \Var(\hat\fpr_i) \frac{n_i^2}{n^2} - \sum_{i=1}^d \frac{n_i}{n}\Var(\hat\fpr^{srs})\\
    % &= \sum_{i=1}^d \textcolor{red}{\frac{\sigma^2_{\fpr_i}}{n_i}} \frac{n_i^2}{n^2} - \sum_{i=1}^d \frac{n_i}{n}\textcolor{red}{\frac{\sigma^2_{\fpr}}{n}}\\
    % &= \sum_{d=1}^d \Var(\hat \fpr)
    %  &= \sum_{i=1}^d \sigma^2_{\fpr_i} \frac{n_i}{n^2} - \sum_{i=1}^d \frac{n_i}{n}\sigma^2_{\fpr}\\
    % &= \frac{1}{n} \sum_{i=1}^d p_i \sigma^2_{\fpr_i} - \frac{1}{n}\sum_{i=1}^d p_i \sigma^2_{\fpr}\\
    % &= \frac{1}{n}\sum_{i=1}^d p_i (  \sigma^2_{\fpr_i} -  \sigma^2_{\fpr})
\end{align}
\textcolor{red}{Complete the computations by looking at the calculations below.}

\paragraph{Simple calculation in the easy setting.}
\begin{gather}
    \Var(\bar{X}_n) = \frac{1}{n}\left[ \Var(\mbbE[X|G]) + \mbbE[\Var(X|G)] \right] \\
    = \frac{1}{n}\left[  \Var(\mu_k) + \mbbE[\mu_k(1-\mu_k)] \right]
\end{gather}

Variance of the proportional sampling:
\begin{equation}
    \frac{1}{n} \sum_{k = 1}^{K} \omega_k \sigma_k^2
    = \frac{1}{n} \sum_{k=1}^{K} \omega_k \mu_k (1 - \mu_k)
\end{equation}


The difference therefore is:
\begin{align}
    &\frac{1}{n}\left[  \Var(\mu_k) + \mbbE[\mu_k(1-\mu_k)] \right] - \frac{1}{n} \sum_{k=1}^{K} \omega_k \mu_k (1 - \mu_k) = \frac{\Var(\mu_k)}{n}
\end{align}

% \[
%     \mu = \sum_{k=1}^{L} \omega_k \mu_k
%     \quad
%     \text{and}
%     \quad
%     ...
% \]


We want to upper bound this by $0$.



The question is how to allocate the observations to keep the variance of the final estimator small?
To answer this question, we have to understand how the variance of the final estimator depends on the allocations.



The motivation for the above estimator is:
\begin{itemize}
    \item The denominator is an estimate for total the ground negatives. We simply count the false negatives in each group and add them up.
    \item The numerator is an estimate for total false positives. We simply count false positives in each group and add them up.
\end{itemize}


Here, we denote by:
\begin{itemize}
    \item $\hat{\fp}$: false positives
    \item $\hat{\tn}$: true negatives
\end{itemize}


\begin{itemize}
    \item Proportion allocation here means allocation according to the ratios in \eqref{eq:weighted-def-fp}
\end{itemize}

Goals here are:

\begin{itemize}
    \item Proportional allocation is better than random allocation
    \item Neyman allocation is better than proportional allocation
\end{itemize}

\subsection*{Generic claim}

Suppose we have parameter of the form:
\[
    \theta = \sum_{k=1}^{K} d_k \theta_k.
\]

Suppose we know the $d_k$ and we have estimator of the form:
\[
    \hat{\theta} = \sum_{k=1}^{K} d_k \hat{\theta}_k.
\]

Assume $d_k$ for $k \in [K]$ are the densities.

We have $n$ samples in total to estimate $\hat{\theta}_k$ for $k \in [K]$.
The question is how to allocate $n_k$ for $k \in [K]$.

A reasonable estimator is such that $\EE[\hat{\theta}_k] \approx \theta_k$.
The goal then is to minimize the variance of the final estimator.

We will consider three strategies to allocate $n$.

\paragraph{Simple random sampling.}

\[
    \Var = \frac{1}{n} \sum_{k=1}^{K} d_k \Var({\hat{\theta}_k}) + \frac{1}{n} \sum_{k=1}^{K} d_k (\EE[\hat{\theta}_k] - \overline{\EE[\hat{\theta}_k]})^2
\]

\paragraph{Proportional sampling.}

\[
    \Var = \frac{1}{n} \sum_{k=1}^{K} d_k \Var({\hat{\theta}}_k).
\]

\paragraph{Neyman sampling.}
\[
    \Var = ...
\]

Difference between simple random sampling and proportional sampling is:
\begin{equation}\label{eq:diff_ps_srs}
\frac{1}{n} \sum_{k=1}^{K} d_k (\EE[\hat{\theta}_k] - \overline{\EE[\hat{\theta}_k]})^2    
\end{equation}


Difference between proportional sampling and optimal sampling is:
\begin{equation}
    \frac{1}{n} \sum_{k=1}^{K} d_k (\Var(\hat{\theta}_k) - \overline{\Var({\hat{\theta}_k})})
\end{equation}



\subsection*{Key ideas}

\begin{itemize}
    \item Write down the estimator for the quantity of interest
    \item Write down the variance of the quantity and how it depends on the allocation
    \item Optimize the allocation to minimize the variance of the estimator
\end{itemize}


\subsection*{Components}

\begin{itemize}
    \item without doing anything, you can do SRS
    \item density estimation: if we do not know this, use an initial step to get some idea of this (for accuracy, this is not required; but for false positive and false negative rates, this will be required)
    \item strata estimation (assume something initially; you see the benefits we get non-homogeneity in either mean or variances)
    \item at this point, you can do proportional
    \item variance estimation: xxx
    \item at this point, you can do Neyman (using the optimal allocation strategy that allocates observations proportional to the product of density and square-root variance
\end{itemize}

\subsection*{Open questions}

\begin{itemize}
    \item defining the stratas: 
        \begin{itemize}
            \item Default: \cite{dalenius1959minimum}
            \item Consider first the simple question of how to define stratas for estimating accuracy
            \item We wil first derive this for accuracy calculation
        \end{itemize}
    \item simultaneous estimation of false positive and false negative rates
    \item handle the case of varying threshold and how to estimate ROC efficiently
\end{itemize}


\subsection*{Constructing strata}

We wish to define strata such that \eqref{eq:diff_ps_srs} is maximized. Thus, we want 
\begin{gather}
    \argmax_{L_1,\dots, L_{K-1}} \sum_{k=1}^K d_k (\mbbE[\hat\theta_k] - \bar{\mbbE[\hat\theta_k]})^2
\end{gather}
where $L_1 < \dots < L_{K-1}$ define the boundaries of the $1, \dots, K-1$ strata on the variable $X$. The $L_k$ for for $k = 1, \dots, K$ affect the objective in the following way:

A part of this calculation is done in \cite{dalenius1959minimum}.
It may not be exactly the same.
We want to understand their analysis so that we can do similar optimization when the parameter is false positive or false negatives rates, rather than the accuracy.
The above is generic, so we may be able to do both in one take.

\subsection*{Comparing the variance under stratified sampling with Neyman allocation vs. sampling with unequal probabilities}

Notation:
\begin{itemize}
    \item $N$: total number of samples in the finite population
    \item $H$: total number of strata (note that $H < N$)
    \item $U_h$: samples falling in stratum $h\in [H]$ (note $\sum_{h = 1}^{H} N_h = N$)
    \item $y_i$ for $i = 1, \dots, N$ are observations
    \item $\theta$ is the unknown scalar parameter
\end{itemize}

Using the results of \citet{clark2022sample}. 

\begin{itemize}
    \item 
    The Horvitz Thompson estimator is 
    \[
    \text{Var}(\hat\theta) \approx \sum_{i=1}^N\sum_{j=1}^N \frac{\pi_{ij} - \pi_i \pi_j}{\pi_i \pi_j}(y_i - \theta)^2
    \]
    where $\pi_i, \pi_j$ for $i, j = 1, \dots, n$ and $\pi_{ij}$ for $i, j = 1, \dots, n$ are given by:
    \[
        \pi_i = ....
        \quad
        \text{and}
        \quad
        \pi_{ij} = ...
    \]

    \item
    Variance of the stratified sampling:
    \[
    \text{Var}(\hat\theta) \approx \sum_{h=1}^H N_h \left(\frac{1}{\pi_h} - 1 \right)S_{h}^2
    \]
    where
    \[
    S_h^2 = \frac{1}{N_h - 1} \sum_{i\in U_h} \left(y_i - \frac{1}{N_h}\sum_{j\in U_h} y_j\right)^2
    \]
    Here $\pi_h$ for $h = 1, \dots, H$ is given by:
    \[
        \pi_h = ...
    \]

    We can rewrite the variance as 
    \begin{align*}
     \text{Var}(\hat\theta) 
     &\approx \sum_{h=1}^H \sum_{i\in U_h} \frac{N_h}{N_h-1} \left(\frac{1}{\pi_h} - 1 \right) \left(y_i - \frac{1}{N_h}\sum_{j\in U_h} y_j\right)^2\\
     &\approx \sum_{h=1}^H \sum_{i\in U_h} \left(\frac{1}{\pi_h} - 1 \right) \left(y_i - \frac{1}{N_h}\sum_{j\in U_h} y_j\right)^2
     % &\approx \sum_{i=1}^N \left( \frac{1}{\pi_i} - 1\right) \left( y_i - \frac{1}{N_h}\sum_{i \in U_h}y_j\right)^2
    \end{align*}
    Using Neyman allocation, we know that the variance-minimizing value for $\pi_h$ is 
    \[
    \pi_h = \frac{S_h N_h}{\sum_{l=1}^H S_l N_l} n 
    \]
    Therefore 
    \[
    \text{Var}(\hat\theta) \approx  \sum_{h=1}^H \sum_{i\in U_h} \left( \frac{1}{\pi_h}  - 1\right)\left( y_i - \theta_h \right)^2 = \sum_{h=1}^H \sum_{i\in U_h} \left( \frac{\sum_{l=1}^H S_l N_l}{S_h N_h}n
    - 1\right)\left( y_i - \theta_h \right)^2
    \]


    \item
    Optimal variance of Poisson without replacement:
    \[
    \text{Var}(\hat\theta) \approx \sum_{i=1}^N \left( \frac{1}{\pi_i} - 1 \right) (y_i-\theta)^2
    \]
    Here, $\pi_i$ for $i = 1, \dots, n$ are given by:
    \[
        \pi_i = ...
    \]
    Hence
    \[
    \text{Var}(\hat\theta) \approx \sum_{h=1}^H \sum_{i\in U_h}  \left( \frac{1}{\pi_i} - 1 \right) \left( y_i-\frac{1}{N}\sum_{i=1}^N y_i\right)^2
    \]
    Now note that 
    \begin{align*}
    &\sum_{i=1}^N (y_i - \theta)^2 \\
    &= \sum_{i=1}^N \left[ (y_i - \theta_h)^2 + (\theta_h - \theta)^2 + 2 (y_i - \theta_h)(\theta_h - \theta)\right] \\
    &= \sum_{i=1}^N \left[ (y_i - \theta_h)^2 + (\theta_h - \theta)^2 \right] + \sum_{h=1}^H (\theta_h - \theta) \sum_{i\in U_h}(y_i - \theta_h) \\
    & = \sum_{i=1}^N \left[ (y_i - \theta_h)^2 + (\theta_h - \theta)^2 \right]
    \end{align*}
    Therefore 
    \begin{align*}
    &\text{Var}(\hat\theta) \\
    &\approx \sum_{h=1}^H \sum_{i\in U_h}  \left( \frac{1}{\pi_i} - 1 \right) \left[ (y_i - \theta_h)^2 + (\theta_h - \theta)^2 \right]\\
    &= \sum_{h=1}^H \sum_{i\in U_h}  \left( \frac{1}{\pi_i} - 1 \right) (y_i - \theta_h)^2 + \sum_{h=1}^H N_h \left( \frac{1}{\pi_i} - 1 \right) (\theta_h - \theta)^2 
    \end{align*}
    We know that the optimal $\pi_i$ under POWOR is given by 
    \[
    \pi_i = \frac{|y_i - \theta|}{\sum_{j=1}^N |y_j - \theta|}n
    \]
    \item For multinomial sampling, we have 
    \begin{align*}
    & \text{Var}(\hat\theta) = \frac{1}{nN^2}\sum_{i=1}^N \pi_i \left( \frac{y_i}{\pi_i} - \sum_{i=1}^N y_i \right)^2\\
    & = \frac{1}{n}\sum_{i=1}^N \pi_i \left( \frac{y_i}{N\pi_i} - \theta \right)^2\\
    % & = \frac{1}{nN^2}\sum_{i=1}^N \frac{y_i^2}{\pi_i} - \frac{\theta^2}{n}
    \end{align*}
    and the optimal $\pi_i$ is given by \citep{imberg2023optimal} (check bc estimator is different)
    \[
    \pi_i = \frac{|y_i - \theta|}{\sum_{j=1}^N|y_j - \theta|}. 
    \]
    
\end{itemize}


In case of the special case with $H=1$, under stratified random sampling we have
\[
\text{Var}(\hat\theta) \approx \sum_{i=1}^n\left( \frac{1}{\pi} - 1\right) (y_i - \theta)^2. 
\]
For Poisson without replacement, we have 
\[
\text{Var}(\hat\theta) \approx \sum_{i=1}^N \left( \frac{1}{\pi_i} - 1 \right) (y_i-\theta)^2. 
\]







\subsection{Other notes}
GREG is a special case of the GREG estimator but under some conditions the two are basically equivalent in large samples \citep{deville1992calibration} %  see https://mathreview.uwaterloo.ca/archive/voli/2/nguyen.pdf
assumption behind calibration is that if the weights perform well for the auxiliary variable they should also perform well for the main variable \citep{wu2001model} (model-calibration estimator)

The reasons for using calibration
are three-fold: \citep{haziza2017construction}
(i) to force consistency of certain survey estimates
to known population quantities;
(ii) to reduce nonsampling errors such as nonresponse errors and coverage errors;
(iii) to improve the precision of estimates.

calibration estimators are designed to be design-based \citep{haziza2017construction} but design-consistent and if the specified model is correct then also model-consistent \citep{kang2007demystifying, chen2017approaches}

GREAT discussion of calibration is also contained in \citep{haziza2017construction}

Three calibration estimators that do not depend on the outcome are 
\begin{itemize}
    \item Hajek 
    \item Ratio estimator 
    \item post-stratified estimator
\end{itemize}
GREG estimator is very efficient when the $y$ is linearly related to $x$ \citep{breidt2017model}
The model-calibration estimator may be more efficient when the relationship between $y$ and $x$ is not linear but the working model does not cover our case
GREG is calibrated over population totals and not over the outcomes, which is pretty cool if we care about multiple variables 

PCA on embeddings to avoid unstable weights
We might need weight trimming. See \citet{haziza2017construction}

still unclear: How does the working model relate to a calibration estimator? to make it model-unbiased? Basically people try to construct estimators that are more efficient if the assumed working model (according to which the estimator has been constructed) is correct


Assuming $m(x_i) = \mathbb{E}[y_i|x_i]$, for large $N_h$, $\mathbb{E}[\Var(\hat\theta_{HT})|\{x_i\}_{i\in \cD}]$ can be approximated as:
\begin{multline}
  \frac{1}{N}\sum_{i=1}^N\mathbb{E}[(y_i - m(x_i))^2] + \frac{1}{N}\sum_{h=1}^H \sum_{i\in \cD_h}\mathbb{E}[(m(x_i) - \bar{m}_h)^2]
\end{multline}
where $m_h:=N_h^{-1}\sum_{i \in \cD_h}m(x_i)$. As the first term is constant, minimizing \Cref{eq:clustering_m} aligns with finding the optimal stratification for $\mathbb{E}[\Var(\hat\theta_{HT})|\bar{x_i}_{i\in \cD}]$ when $m\equiv \hat{m}$. 


If $m(x)=\mathbb{E}[y|x]$, then this objective is approximately equal to % TODO: not true
\begin{gather}
    (y_i - \theta_h)^2 = (y_i - m(x_i) + m(x_i) - \theta_h)^2 \\
    = (y_i - m(x_i))^2 + (m(x_i) - \theta_h)^2 + 2(y_i - m(x_i))(m(x_i) - \theta_h)\\
    = (y_i - m(x_i))^2 + (m(x_i) - m_h + m_h - \theta_h)^2 + 2(y_i - m(x_i))(m(x_i) - \theta_h)\\
    = (y_i - m(x_i))^2 + (m(x_i) - m_h)^2 + (m_h - \theta_h)^2 + 2(m(x_i) - m_h)(m_h-\theta_h) + 2(y_i - m(x_i))(m(x_i) - \theta_h) 
\end{gather}
Now note that the last term is $0$ by the law of total expectation and the fact that $\mathbb{E}[y_i] = m(x_i)$. In addition, 
\begin{align}
   &  \mathbb{E}[(m(x_i) - m_h)(m_h - \theta_h)] \\
   &  = \mathbb{E}[m(x_i)m_h + m_h^2 - m(x_i)\theta_h - m_h\theta_h]\\
    & = \frac{1}{N_h}\sum_{j=1}^{N_h}\mathbb{E}\left[m(x_i)m(x_j)\right] +  
    \frac{1}{N_h^2} \sum_{j=1}^{N_h}\sum_{l=1}^{N_h}\mathbb{E}[m(x_j) m(x_l)] 
    - \frac{1}{N_h}\sum_{j=1}^{N_h}\mathbb{E}[m(x_i)y_j] - \frac{1}{N_h^2} \sum_{j=1}^{N_h}\sum_{l=1}^{N_h}\mathbb{E}[m(x_j) y_l]\\
    & = \frac{1}{N_h}\sum_{j=1}^{N_h}\mathbb{E}\left[m(x_i)m(x_j)\right] +  
    \frac{1}{N_h^2} \sum_{j=1}^{N_h}\sum_{l=1}^{N_h}\mathbb{E}[m(x_j) m(x_l)] 
    - \frac{1}{N_h}\sum_{j=1}^{N_h}\mathbb{E}[m(x_i)m(x_j)] - \frac{1}{N_h^2} \sum_{j=1}^{N_h}\sum_{l=1}^{N_h}\mathbb{E}[m(x_j) m(x_l)]\\
    & = 0.
\end{align}
where we used the law of total expectation in the second-to-last equality. 

Thus, it follows that 
\begin{align}
    & \mathbb{E}[(y_i - m(x_i))^2 + (m(x_i) - m_h)^2 + (m_h - \theta_h)^2 + 2(m(x_i) - m_h)(m_h-\theta_h) + 2(y_i - m(x_i))(m(x_i) - \theta_h)] \\
    & =  \mathbb{E}[(y_i - m(x_i))^2 + (m(x_i) - m_h)^2 + (m_h - \theta_h)^2]
\end{align}
Note that 
\begin{gather}
\mathbb{E}[(m_h - \theta_h)^2] = \mathbb{E}\left[ \left(\frac{1}{N_h}\sum_{i=1}^{N_h}(y_i - m(x_i))\right)^2\right] \\
= \frac{1}{N_h^2}\sum_{i=1}^{N_h}\mathbb{E}[(y_i - m(x_i))^2] + \frac{1}{N_h}\sum_{i=1}^{N_H}\sum_{j=1, j\neq i}^{N_h}\mathbb{E}[(y_i - m(x_i))(y_j - m(x_j))] \\
= \frac{1}{N_h^2}\sum_{i=1}^{N_h} \mathbb{E}[(y_i - m(x_i))^2] \approx 0
\end{gather}
for large $N_h$ because of the independence of the observations and the fact that $|y_i - m(x_i)|$ is bounded. Thus we have 
\begin{gather}
    \mathbb{E}[(y_i - m(x_i))^2 + (m(x_i) - m_h)^2 + (m_h - \theta_h)^2]\\
    \approx \mathbb{E}[(y_i - m(x_i))^2] + \mathbb{E}[(m(x_i) - m_h)^2]
\end{gather}


% Now we take the expectation and obtain 
% \begin{gather}
%     \mathbb{E}[(y_i - m(x_i))^2] + \mathbbE[(m(x_i) - m_h)^2] + \mathbb{E}[(m_h - \theta_h)^2] + 2\mathbbE[(m(x_i) - m_h)(m_h-\theta_h)] + 2\mathbb{E}[(y_i - m(x_i))(m(x_i) - \theta_h)]\\
%     = 
% \end{gather}


% For $N_h$ large enough, $m_h - \theta_h \approx 0$ hence 
% \begin{gather}
%     = (y_i - m(x_i))^2 + (m(x_i) - m_h)^2 + 2(y_i - m(x_i))(m(x_i) - \theta_h) \\
%     = 
% \end{gather}

% \begin{gather}
%     \frac{1}{N_h} \sum_{i=1}^{N_h} y_i m(x_i) - m(x_i)^2 + m(x_i)\theta_h - y_i\theta_h\approx m_h\theta_h - \frac{1}{N}\sum_{i=1}^{N_h}m(x_i)^2 + \theta_h m_h - \theta_h^2 \approx - \frac{1}{N}\sum_{i=1}^{N_h} m(x_i)^2 + m_h^2
% \end{gather}
